Analysis of Non-local Multicontinuum Upscaling for Dual Continuum Model

In this paper, we develop and analyze a rigorous multiscale upscaling method for dual continuum model, which serves as a powerful tool in subsurface formation applications. Our proposed method is capable of identifying different continua and capturing non-local transfer and effective properties in the computational domain via constructing localized multiscale basis functions. The construction of the basis functions consists of solving local problems defined on oversampling computational region, subject to the energy minimizing constraints that the mean values of the local solution are zero in all continua except for the one targeted. The basis functions constructed are shown to have good approximation properties. It is shown that the method has a coarse mesh dependent convergence. We present some numerical examples to illustrate the performance of the proposed method.

==> method_description.tex <==
% !TeX spellcheck = en_US
In this section, we will describe our proposed method in detail. 
To start with, we introduce the concepts of coarse and fine meshes. 
We start with a plain partition of calculation domain $\Omega$, $\mesh^H$. 
This partition is called a coarse mesh, which does not necessarily resolve any multiscale features. 
We denote one element in $\mesh^H$ as $K$ and name it as a coarse element. 
Here, $H>0$ is the coarse mesh size. 
We denote the number of coarse elements and coarse grid nodes as $N$ and $N_c$ respectively. 
The collection of all coarse element edges is called $\edge^H$. 
To sufficiently resolve the solution, we refine the coarse mesh $\mesh^H$ into a fine mesh $\mesh^h$, where $h>0$ is called the fine mesh size. 
We remark that the fine grid system is only used in locally solving process, where all local problems are solved continuously. 
Therefore, we don't consider fine grid in our analysis hereinafter. 
A demonstration of coarse and fine meshes is given in Figure~\ref{fig:mesh}. 

\begin{figure}[ht!]
\centering
\subimport{../}{multiscale.tex}
\caption{An illustration of the coarse and fine meshes.}
\label{fig:mesh}
\end{figure}

Next, we clarify more notions concerning every coarse element. 
Letting $K_j \in \mesh^H$ be the $j$-th coarse element, an oversampling domain $\osdomain{j}$ is defined by expanding $K_j$ with $m$ layers of coarse elements in $\Omega$. 
An illustration is given in Figure~\ref{fig:osdomain}. 
Moreover, similar to the partition of computational domain $\Omega$, for $i = 1,2$, we denote $K_j = \cup_{l=1}^{L_i^{(j)}} \kij{l}{i,j}$, where $L_i^{(j)}$ denotes the number of high conductive channels plus matrix within $K_j$ for continua $i$. 

\begin{figure}[ht!]
\centering
\subimport{../}{oversampling.tex}
\caption{An illustration of oversampling domain.}
\label{fig:osdomain}
\end{figure}

We now proceed to describing the proposed method step by step. 

\textbf{Step 1. Definition of auxiliary basis functions.} 
Within $K_j$($j = 1,\ldots, N$), for each $l = 1,\ldots, L_i^{(j)}$, we directly define our auxiliary basis function $\auxbasis{l}{i,j} \in P^0(\mesh^h(\osdomain{j}))$, where $\mesh^h(\osdomain{j})$ denotes the restriction of $\mesh^h$ on $\osdomain{j}$, as 
\begin{equation}
	\auxbasis{l}{i,j} = \dfrac{1}{|K_l^{(i,j)}|}\mathcal{I}_{\kij{l}{i,j}}.
	\label{eq:auxbasis}
\end{equation}
Here, 
$|\kij{l}{i,j}|$ denotes the area of $\kij{l}{i,j}$ and 
$\mathcal{I}_{\kij{l}{i,j}}$ is the characteristic function.  
The local auxiliary space for continua $i$ is constructed as
\begin{equation}
	\aux^{(i,j)} = \mathrm{span}\{\auxbasis{l}{i,j} |1\leq l\leq L_i^{(j)}\}.
\end{equation}
Furthermore, we define the local auxiliary space as
\begin{equation}
\aux^j = \aux^{(1,j)}\times\aux^{(2,j)}.
\end{equation}
%We remark that each basis function in the local auxiliary space represents a continua. 
The global auxiliary space is defined as the direct sum of all local auxiliary spaces as 
\begin{equation}
	\aux = \oplus_{j = 1}^N \aux^j.
\end{equation}

\textbf{Step 2. Construction of multiscale basis functions.} 
For the convenience of describing the method and the subsequent convergence analysis, for all $v = (v_1,v_2)\in \lsquare{K_j}$, we introduce a local projection operator $\pi_j:\lsquare{K_j}\rightarrow\aux$ as
\begin{equation}
\pi_j(v) = 
\left(
\sum_{l = 1}^{L_1^{(j)}}(v_1,\auxbasis{l}{1,j})\auxbasis{l}{1,j},
\sum_{l = 1}^{L_2^{(j)}}(v_2,\auxbasis{l}{2,j})\auxbasis{l}{2,j}
\right)
\end{equation}
and a global projection operator $\pi: \lsquare{\Omega}\rightarrow\aux$ is defined as 
\begin{equation}
\pi(v) = \sum_{j=1}^N\pi_j(v),\quad \forall v \in \lsquare{\Omega}.
\label{eq:basis_proj}
\end{equation}

The local multiscale basis functions are constructed by the following variational form of minimization problem. 
Within the oversampling domain $\osdomain{j}$ of every $K_j\subset \Omega$, find $\msbasis{l}{i,j} \in V(\osdomain{j})$ and $\overline{T}^{i,j,l}_{i',j',l'} \in \R$ such that for $i=1,2$, we have
\begin{equation}
	\begin{split}
	a_Q(\msbasis{l}{i,j},w)+ \sum_{i'=1}^2\sum_{\kij{l'}{i',j'}\subset\osdomain{j}}\overline{T}^{i,j,l}_{i',j',l'}(w\cdot \unit{i'},\auxbasis{l'}{i',j'}) & = 0, \quad \forall w\in V(\osdomain{j}),\\
	(\msbasis{l}{i,j}\cdot \unit{i'},\auxbasis{l'}{i',j'}) &= \delta_{i,i'}\delta_{l, l'}\delta_{j, j'},\quad \forall \kij{l'}{i',j'}\subset\osdomain{j}.
	\end{split}
	\label{eq:ms_min}
\end{equation}
Here, $\unit{i}$ is the canonical basis for $\R^2$. 
$\delta_{i,i'}$, $\delta_{l, l'}$ and $\delta_{j, j'}$ are the delta Dirac function. 
We use the local multiscale basis functions to obtain the multiscale finite element space, which will be used for deriving the multiscale solution, as 
\begin{equation}
	\msspace = \mathrm{span}\{\msbasis{l}{i,j} |1\leq l\leq L_i^{(j)}, 1\leq j \leq N, i = 1,2\}.
\end{equation}

The local multiscale basis functions are inspired from the global multiscale basis functions which are constructed in the similar way but on the global domain. For every coarse element $K_j$ in $\Omega$, find $\globasis{l}{i,j}\in V$ and $T^{i,j,l}_{i',j',l'}\in\R$ such that
\begin{equation}
	\begin{split}
	a_Q(\globasis{l}{i,j},w)+ \sum_{i'=1}^2\sum_{\kij{l'}{i',j'}\subset\Omega}T^{i,j,l}_{i',j',l'}(w\cdot \unit{i'},\auxbasis{l'}{i',j'}) & = 0, \quad \forall w\in V,\\
	(\globasis{l}{i,j}\cdot \unit{i'},\auxbasis{l'}{i',j'}) &= \delta_{i,i'}\delta_{l, l'}\delta_{j, j'},\quad \forall \kij{l'}{i',j'}\subset\Omega.
	\end{split}
	\label{eq:glo_min}
\end{equation}
The global multiscale finite element space is thus defined as
\begin{equation}
	\glo = \mathrm{span}\{\globasis{l}{i,j} | 1\leq l\leq \lij, 1\leq j \leq N, i = 1,2\}.
\end{equation}
As our analysis suggest, the global basis functions exhibit exponential decay properties and have small values outside a sufficiently large oversampling region. The fact suggests that we can save computational costs by localizing the basis functions by truncating the domain, without introducing huge error. 

We remark that if we denote $\tilde{V}$ as the null space of the global projection operator $\pi$, for any $\globasis{l}{i,j}\in \glo$, we have
\begin{equation}
	a_Q(\globasis{l}{i,j},v) = 0, \quad \forall v\in\tilde{V}.
\end{equation}
This implies that with respect to the inner product of $a_Q$, $\tilde{V}\subset \glo^{\bot}$. 
As a matter of fact, $\tilde{V} = \glo^{\bot}$.
 
\textbf{Step 3. Multiscale solution.} 
The process of finding the multiscale solution can be described as follows. 
Find $p_{\text{ms}} = (p_{\text{ms},1}, p_{\text{ms},2})$ with $p_{\text{ms}}(t,\cdot) \in \msspace$ s.t. for all $v = (v_1, v_2)$ with $v(t, \cdot) \in \msspace$,
\begin{equation}
c \left(\dfrac{\partial p_{\text{ms}}}{\partial t}, v \right) + a_Q(p_{\text{ms}}, v) = (f,v).
\label{eq:sol_ms}
\end{equation}
 


==> multiscale.tex <==
\begin{tikzpicture}[scale = 1.2]
	\draw[step=1cm,black,thick] (-2.14,-2.14) grid (2.14,2.14);
	\draw[step=0.1cm, gray, very thin] (-2.14,-2.14) grid (2.14,2.14);
	\draw[blue,thick] (0,0) rectangle (1,-1);
	\path[red,-stealth] (1,-0.5) edge[bend left] (3,-0.5);
	\draw[blue,thick] (3,0) rectangle (4.5,-1.5);
	\draw[step=0.15cm, gray, very thin] (3,0) grid (4.5,-1.5);
	\draw[red,thin] (3.6,-0.6) rectangle (3.75, -0.75);
	\draw (3.75,0.25) node(K) [draw=white] {$K$};
	
\end{tikzpicture}


==> numerical_example.tex <==
% !TeX spellcheck = en_US

In this section, we present two numerical examples with high-contrast media to 
verify the convergence of our proposed method,  
using a fine-scale approximation $p_{\text{f}}$ as a reference solution. 
We will compute the coarse cell average $\meansol_{\text{f}}$ of 
the fine-scale solution $p_{\text{f}}$ and $\meansol_{\text{ms}}$ of the multiscale solution $p_{\text{ms}}$, and
compare the relative $L_2$ error of coarse cell average, i.e. 
\begin{equation}\label{eq:error}
	e_{L_2}^{(i)} = \|\meansol_{\text{f},i}-\meansol_{\text{ms},i}\|_{L^2},
	\qquad \|\meansol_{\text{f},i}-\meansol_{\text{ms},i}\|^2_{L_2} = \dfrac{\sum_K(\meansol^K_{\text{f},i}-\meansol_{\text{ms},i}^K)^2}{\sum_K(\meansol^K_f)^2},
	\qquad \meansol_{\text{f},i}^K = \dfrac{1}{|K|}\int_K p_{\text{f},i} \dif x. 
\end{equation}
In all the experiments, we take the spatial domain to be $\Omega = (0,1)^2$ and 
the fine mesh size to be $h = 1/256$. 
%We will also see the effects of the contrast values of the media on the error, 
%while the configurations of the media remain unchanged. 
An example of the media $\kappa_1$ and $\kappa_2$ used in the experiments is illustrated in Figure~\ref{fig:kappa1}. 
In the figure, the contrast values, i.e. the ratio of the maximum and the minimum in $\Omega$, of the media are
$\overline{\kappa}_1 = \overline{\kappa}_2 = 10^4$. 
Unless otherwise specified, we set $\sigma = 1$.

\begin{figure}[!ht]
	\centering
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width=.9\linewidth]{k1_256}
		\caption{$\kappa_1$}
	\end{subfigure}
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{k2_256}
		\caption{$\kappa_2$}
	\end{subfigure}
\caption{High contrast permeability field}
\label{fig:kappa1}
\end{figure}

\subsection{Experiment 1 static case}
In this experiment, we consider the dual continuum model under steady state
\begin{equation}
\begin{split}
 - \text{div}(\kappa_1 \nabla p_1) + \sigma(p_1 - p_2) = f_1, \\
 - \text{div}(\kappa_2 \nabla p_2) - \sigma(p_1 - p_2) = f_2. 
\end{split}
\label{eq:ss}
\end{equation} 
The source terms are given as $f_1(x,y) = 1$ and $f_2(x,y)$ as shown in Figure~\ref{fig:f2_static}. 
In Figure~\ref{fig:sol_static}, we plot the fine-scale solution, the coarse-scale average 
and the NLMC coarse-scale solution with coarse mesh size $H = 1/64$ and number of oversampling layers $m = 8$, 
from which we observe very good agreement between the coarse-scale average and the NLMC solution.
In Table~\ref{tab:conv_static}, we present the relative $L^2$ error with varying coarse grid size. 
With the number of oversampling layers satisfying the sufficient condition, 
we can see that the error converges. 
We also compare the performance of different numbers of oversampling layers under fixed coarse mesh size $H$. 
The results are summarized in Table~\ref{tab:error_32} for $H = 1/32$ and Table~\ref{tab:error_64} for $H = 1/64$. 
It can be seen that the error decays quickly with respect to the number of oversampling layers $m$ for both cases, 
which verifies the fact that the oversampling region has to be sufficiently large to obtain quality numerical approximations. 
\begin{figure}[!ht]
	\centering
	\includegraphics[width = .45\linewidth]{static_f2}
	\caption{Source term $f_2$ in Experiment 1.}
	\label{fig:f2_static}
\end{figure}

%\begin{figure}[!ht]
%	\label{fig:sol_static}
%	\centering
%	\begin{subfigure}{.32\textwidth}
%		\centering
%		\includegraphics[width = .9\linewidth]{static_fine_1}
%	\end{subfigure}
%	\begin{subfigure}{.32\textwidth}
%		\centering
%		\includegraphics[width = .9\linewidth]{static_nlmc_coarse_1}
%	\end{subfigure}
%	\begin{subfigure}{.32\textwidth}
%		\centering
%		\includegraphics[width = .9\linewidth]{static_nlmc_fine_1}
%	\end{subfigure}
%
%
%	\begin{subfigure}{.32\textwidth}
%		\centering
%		\includegraphics[width = .9\linewidth]{static_fine_2}
%	\end{subfigure}
%	\begin{subfigure}{.32\textwidth}
%		\centering
%		\includegraphics[width = .9\linewidth]{static_nlmc_coarse_2}
%	\end{subfigure}
%	\begin{subfigure}{.32\textwidth}
%		\centering
%		\includegraphics[width = .9\linewidth]{static_nlmc_fine_2}
%	\end{subfigure}
%\caption{Numerical results for static cases. Coarse mesh size $1/64$. Top row: first continuum. Bottom: second continuum. First column: fine-scale solution. Second column: coarse-scale solution by NLMC. Third column: fine-scale solution reconstructed from NLMC.}
%\end{figure}

\begin{figure}[!ht]
	\centering
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{static_fine_1}
	\end{subfigure}
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{static_fine_2}
	\end{subfigure}

	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{static_fine_upscale_1}
	\end{subfigure}
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{static_fine_upscale_2}
	\end{subfigure}
	
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{static_nlmc_coarse_1}
	\end{subfigure}
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{static_nlmc_coarse_2}
	\end{subfigure}

	\caption{Plots of the numerical approximations of pressure with coarse mesh size $H=1/64$ and $m = 8$ oversampling layers in Experiment 1. 
	Left: first continuum. Right: second continuum. First row: fine-scale solution. Second row: coarse-scale average of fine-scale solution. Third row: NLMC solution.}
	\label{fig:sol_static}
\end{figure}

\begin{table}[!ht]
	\centering
	\begin{tabular}{c |c| c| c}
		\hline
%		\multirow{2}{*}{	$H$} &\multirow{2}{*} {$m$} &\multicolumn{2}{|c|}{$e_{L_2}$ by continuum} & \multirow{2}{*} {$e_{a_Q}$}\\
%		\cline{3-4}
%		 & & 1st & 2nd & \\
		$H$ & $m$ & $e_{L^2}^{(1)}$ & $e_{L^2}^{(2)}$\\
%		 & $e_{a_Q}$ \\
		\hline
		1/8 & 3 & 96.7318\% & 88.9818\% \\
%		& 95.4984\% \\
		1/16 & 5 & 32.3229\% & 19.3473\% \\
%		& 41.9306\% \\
		1/32 & 6 & 0.6045\% & 0.3680\%\\
%		 &6.3708\%  \\
%		1/64 & 7 & 0.7959\% & 0.4219\%&  6.0724\% \\
		1/64 & 8 & 0.0550\% & 0.0296\% \\
%		& 1.6930\%\\
%		1/32 & 7 & 0.0403\% & 0.0246\% & 2.3095\%\\
%		1/64 & 9 & 0.0017\% & 0.0018\% & 0.3975\%\\
		\hline
	\end{tabular}
	\caption{Convergence of $e_{L_2}$ with respect to coarse mesh size $H$ in Experiment 1.}
	\label{tab:conv_static}
\end{table}

\begin{table}[!ht]
	\centering
	\begin{tabular}{c|c|c|c}
		\hline
		$m$ & Area Ratio & $e_{L^2}^{(1)}$ & $e_{L^2}^{(2)}$\\
		\hline
%		1 & 0.88\% & 99.9831 & 98.9553 \\
%		2 & 2.44\% & 99.8920 & 97.7704 \\
		3 & 4.79\% & 99.3677\% & 93.9357\% \\
		4 & 7.91\% & 76.6083\% & 55.1631\% \\
		5 & 11.81\% & 8.6605\% & 5.3115\% \\
		6 & 16.50\% & 0.6045\% & 0.3680\% \\
		\hline
	\end{tabular}
	\caption{Comparison of $e_{L_2}$ error with different number of oversampling layers $m$ for $H=1/32$ in Experiment 1.}
	\label{tab:error_32}
\end{table}
\begin{table}[!ht]
	\centering
	\begin{tabular}{c|c|c|c}
		\hline
		$m$ & Area Ratio & $e_{L^2}^{(1)}$ & $e_{L^2}^{(2)}$\\
		\hline
%		1 & 0.22\%  & 99.9976 & 99.5167 \\
		2 & 0.61\% & 99.9102\% & 97.9631\% \\
		4 & 1.98\% & 99.1268\% & 91.9240\% \\
		6 & 4.13\% & 11.8898\% & 6.3181\% \\
		7 & 5.49\% & 0.7959\% & 0.4219\% \\
		8 & 7.06\% & 0.0550\% & 0.0296\% \\
		\hline
	\end{tabular}
	\caption{Comparison of $e_{L_2}$ error with different number of oversampling layers $m$ for $H=1/64$ in Experiment 1.} 
	\label{tab:error_64}
\end{table}
%\begin{table}[!ht]
%	\centering
%	\begin{tabular}{c c c c}
%		\hline
%		$H$ & $m$ & 1st continuum & 2nd continuum\\
%		\hline
%		1/8 & 3 & 96.7274\% & 89.2802\% \\
%		1/16 & 5 & 32.3260\% & 19.3434\% \\
%		1/32 & 6 & 0.6050\% & 0.3720\% \\
%		1/64 & 7 & 0.7959\% & 0.4223\% \\
%		1/64 & 8 & 0.0550\% & 0.0310\% \\
%		1/32 & 7 & 0.0403\% & 0.0628\% \\
%		1/64 & 9 & 0.0017\% & 0.0019\% \\
%		\hline
%	\end{tabular}
%	\caption{$e_2$ of static cases}
%\end{table}

\subsection{Experiment 2: time-dependent case}
The time dependent case faces the similar issue with the error. $f_1(x,y) = 1$ and $f_2(x,y)$ is 
depicted in Figure~\ref{fig:source_time}, which represents a simplified five-spot well rate. 
The temporal domain is $[0, T]$ with final time $T= 5$.
In Figure~\ref{fig:sol_time}, we plot the fine-scale solution, the coarse-scale average 
and the NLMC coarse-scale solution with coarse mesh size $H = 1/64$ and number of oversampling layers $m = 8$. 
Again, the NLMC solution is a good approximation for the coarse-scale average. 
In Figure~\ref{fig:evolve_time}, we depict the change of pressure at different time steps. 
In Table~\ref{tab:conv_time}, we present the relative $L^2$ error with varying coarse grid size. 
Again, with the number of oversampling layers satisfying the sufficient condition, 
we can see that the error converges very well. 

\begin{figure}[!ht]
	\centering
	\includegraphics[width = .45\linewidth]{five_well}
	\caption{Source term $f_2$ in Experiment 2.}
	\label{fig:source_time}
\end{figure}

\begin{figure}[!ht]
	\centering
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{time_fine_1_20}
	\end{subfigure}
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{time_fine_2_20}
	\end{subfigure}
	
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{time_fine_upscale_1_20}
	\end{subfigure}
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{time_fine_upscale_2_20}
	\end{subfigure}
	
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{time_nlmc_coarse_1_20}
	\end{subfigure}
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{time_nlmc_coarse_2_20}
	\end{subfigure}
	\caption{Plots of the numerical approximations of final-time pressure with coarse mesh size $H=1/64$ and $m = 8$ oversampling layers in Experiment 2. 
	Left: first continuum. Right: second continuum. First row: fine-scale solution. Second row: coarse-scale average of fine-scale solution. Third row: NLMC solution.}
	\label{fig:sol_time}
\end{figure}


\begin{table}[!ht]
	\centering
	\begin{tabular}{c |c| c| c}
		\hline
%		\multirow{2}{*}{	$H$} &\multirow{2}{*} {$m$} &\multicolumn{2}{|c|}{$e_{L_2}$ by continuum} & \multirow{2}{*} {$e_{a_Q}$}\\
%		\cline{3-4}
%		& & 1st & 2nd & \\
		$H$ & $m$ & $e_{L^2}^{(1)}$ & $e_{L^2}^{(2)}$ \\
%		& $e_{a_Q}$ \\
		\hline
		1/8 & 3 & 20.6422\% & 58.4975\%\\
%		 & 85.5185\% \\
		1/16 & 5 & 1.1245\% & 2.6226\%\\
%		 & 60.7209\%\\
		1/32 & 6 & 0.0254\% & 0.0717\%\\
%		 & 23.1083\%\\
%		1/64 & 7 & 0.0307\% & 0.0217\% & 18.1244\%\\
		1/64 & 8 & 0.0017\% & 0.0037\%\\
%		 & 5.0113\%\\
%		1/32 & 7 & 0.0015\% & 2.4280e-6 & 45.0902\%\\
%		1/64 & 9 & 1.4495e-6 & 1.0240e-6 & 18.1012\% \\
		\hline
	\end{tabular}
	\caption{Convergence of $e_{L_2}$ with respect to coarse mesh size $H$ in Experiment 2.}
	\label{tab:conv_time}
\end{table}

\begin{figure}[!ht]
	\centering
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{time_nlmc_coarse_1_5}
	\end{subfigure}
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{time_nlmc_coarse_2_5}
	\end{subfigure}
	
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{time_nlmc_coarse_1_10}
	\end{subfigure}
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{time_nlmc_coarse_2_10}
	\end{subfigure}
	
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{time_nlmc_coarse_1_20}
	\end{subfigure}
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width = .9\linewidth]{time_nlmc_coarse_2_20}
	\end{subfigure}
	\caption{Plots of the NLMC numerical approximations of pressure at various time instants with coarse mesh size 
	$H=1/64$ and $m = 8$ oversampling layers in Experiment 2. 
	Left: first continuum. Right: second continuum. First row: $t = 1.25$. Second row: $t = 2.5$. Third row: $t = 5$.}
	\label{fig:evolve_time}
\end{figure}

%\begin{table}[!ht]
%	\centering
%	\begin{tabular}{c c c c}
%		\hline
%		$H$ & $m$ & 1st continuum & 2nd continuum\\
%		\hline
%		1/8 & 3 & 41.4342\% & 42.5359\% \\
%		1/16 & 5 & 1.6167\% & 19.1192\% \\
%		1/32 & 6 & 0.1663\% & 9.4997\% \\
%		1/64 & 7 & 0.0366\% & 2.1412\% \\
%		1/64 & 8 & 0.0203\% & 2.1416\% \\
%		1/32 & 7 & 0.1646\% & 9.4996\% \\
%		1/64 & 9 & 0.0203\% & 2.1416\%\\
%		\hline
%	\end{tabular}
%	\caption{$e_2$ of time-dependent cases}
%\end{table}




==> oversampling.tex <==
\begin{tikzpicture}[scale = 1.2]
	\draw[step=0.5cm,black,thick] (-1.15,-1.65) grid (2.15,1.65);
	\draw[step=0.1cm, gray, very thin] (-1.15,-1.65) grid (2.15,1.65);
	\draw[blue,very thick] (0,-1) rectangle (1.5,0.5);
	\draw[red,thick] (0.5,-0.5) rectangle (1,0);
	
	\path[red,-stealth] (1.5,-0.5) edge[bend right] (3,-0.5);
	\draw[blue,very thick] (3,0.75) rectangle (5.25,-1.5);
	\draw[step=0.15cm, gray, very thin] (3,0.75) grid (5.25,-1.5);
	\draw[step=0.75cm, black,thick] (3,0.75) grid (5.25,-1.5);
	\draw[red,thick] (3.75,-0.75) rectangle (4.5, 0);
	\draw (5,1.5) node(x) [draw=white] {\begin{tabular}{c}Oversampling domain\\ with 1 layer, $K_{i,1}$\end{tabular}};
	
	\draw (4.1,-0.4) node(ki){$K_i$};
	
\end{tikzpicture}
